Stylizing 3D Scene via Implicit Representation and HyperNetwork

In this work, we aim to address the 3D scene stylization problem - generating stylized images of the scene at arbitrary novel view angles. A straightforward solution is to combine existing novel view synthesis and image/video style transfer approaches, which often leads to blurry results or inconsistent appearance. Inspired by the high-quality results of the neural radiance fields (NeRF) method, we propose a joint framework to directly render novel views with the desired style. Our framework consists of two components: an implicit representation of the 3D scene with the neural radiance fields model, and a hypernetwork to transfer the style information into the scene representation. In particular, our implicit representation model disentangles the scene into the geometry and appearance branches, and the hypernetwork learns to predict the parameters of the appearance branch from the reference style image. To alleviate the training difficulties and memory burden, we propose a two-stage training procedure and a patch sub-sampling approach to optimize the style and content losses with the neural radiance fields model. After optimization, our model is able to render consistent novel views at arbitrary view angles with arbitrary style. Both quantitative evaluation and human subject study have demonstrated that the proposed method generates faithful stylization results with consistent appearance across different views.

==> draft.tex <==
1-1 好的，我們會重新輸出影片 (使用不同 codec e.g. mp4)，確認每個撥放器都沒問題

1-2 在比較 consistent 的部分，我們 render 的 novel view 是基於 Tanks and Temples dataset 裡面各個場景的 testing view，在計算 consistency score 的時候會比較公平 (view間的間隔是由dataset決定的)。我們可以對 testing novel views 做角度的interpolation 以創造出更密集的frame，但這樣 long consistency 的設定 (t, t-7) 兩個 frame 的距離就縮短了，那這樣的話對 video style transfer 的 method 來說就變簡單了，感覺會不太公平?

2. 關於 某r 提到的 variable/notation 沒有定義清楚，以他舉的例子 F{base}, F{geo}, F{app} are not properly introduced. 我們在 WACV PDF line 321-350 其實本來就有分別解釋他們的作用，目前 paper 的版本我們也讀過，我們覺得 notation 都算清楚，感覺只是個案？

3-1. OK, 已換
3-2. 已改，請曾博再看一下

